Bridging the Information Gap Between Domain-Specific Model and General LLM for Personalized Recommendation

Generative large language models(LLMs) are proficient in solving general problems but often struggle to handle domain-specific tasks. This is because most of domain-specific tasks, such as personalized recommendation, rely on task-related information for optimal performance. Current methods attempt to supplement task-related information to LLMs by designing appropriate prompts or employing supervised fine-tuning techniques. Nevertheless, these methods encounter the certain issue that information such as community behavior pattern in RS domain is challenging to express in natural language, which limits the capability of LLMs to surpass state-of-the-art domain-specific models. On the other hand, domain-specific models for personalized recommendation which mainly rely on user interactions are susceptible to data sparsity due to their limited common knowledge capabilities. To address these issues, we proposes a method to bridge the information gap between the domain-specific models and the general large language models. Specifically, we propose an information sharing module which serves as an information storage mechanism and also acts as a bridge for collaborative training between the LLMs and domain-specific models. By doing so, we can improve the performance of LLM-based recommendation with the help of user behavior pattern information mined by domain-specific models. On the other hand, the recommendation performance of domain-specific models can also be improved with the help of common knowledge learned by LLMs. Experimental results on three real-world datasets have demonstrated the effectiveness of the proposed method.

==> Tables/ablation.tex <==
\begin{table*}[t]\small
\centering
\tabcolsep=0.18cm
\begin{tabular}{lcccccccccccc}
\toprule
Interaction Predict & \multicolumn{4}{c}{ML-1M} & \multicolumn{4}{c}{Grocery} & \multicolumn{4}{c}{Health} \\
Models & acc & prec & rec & f1 & acc & prec & rec & f1 & acc & prec & rec & f1 \\
\midrule
LLM-UIToken      & 0.770 & 0.826 & 0.684 & 0.748 & 0.695 & 0.753 & 0.579 & 0.655 & 0.677 & 0.768 & 0.506 & 0.610 \\
LLM-NCF          & 0.794 & 0.845 & 0.719 & 0.777 & 0.715 & 0.785 & 0.592 & 0.675 & 0.694 & 0.769 & 0.556 & 0.645 \\
LLM-LGCN         & 0.805 & 0.858 & 0.732 & 0.790 & 0.731 & 0.790 & 0.628 & 0.700 & 0.708 & 0.775 & 0.587 & 0.668 \\
\midrule
NCF-LLM          & 0.801 & 0.823 & 0.767 & 0.794 & 0.712 & 0.763 & 0.615 & 0.681 & 0.701 & 0.761 & 0.584 & 0.661 \\
LGCN-LLM         & 0.809 & 0.804 & 0.819 & 0.811 & 0.721 & 0.774 & 0.625 & 0.692 & 0.711 & 0.761 & 0.616 & 0.681 \\
\midrule
BDLM-NCF-LLM     & 0.801 & 0.839 & 0.745 & 0.789 & 0.714 & 0.776 & 0.600 & 0.677 & 0.695 & 0.767 & 0.561 & 0.648 \\
BDLM-LGCN-LLM    & 0.810 & 0.847 & 0.758 & 0.799 & 0.704 & 0.754 & 0.605 & 0.671 & 0.699 & 0.746 & 0.604 & 0.678 \\
BDLM-NCF-DRS     & 0.805 & 0.821 & 0.780 & 0.800 & 0.716 & 0.773 & 0.611 & 0.683 & 0.702 & 0.763 & 0.588 & 0.664 \\
BDLM-LGCN-DRS    & 0.815 & 0.812 & 0.819 & 0.816 & 0.725 & 0.777 & 0.631 & 0.697 & 0.716 & 0.750 & 0.616 & 0.681 \\

\bottomrule

\end{tabular}

\caption{Main results on MovieLens-1M, Amazon-Grocery and Amazon-Health test sets for interaction prediction task.}
\label{tab:ablation}
\end{table*}

==> Tables/main-res.tex <==
% \begin{table*}[t]
% \centering
% \begin{tabular}{lcccccccccccc}
% \toprule
% Interaction Predict & \multicolumn{4}{c}{ML-1M} & \multicolumn{4}{c}{Grocery} & \multicolumn{4}{c}{Health} \\
% Models & acc & prec & rec & f1 & acc & prec & rec & f1 & acc & prec & rec & f1 \\
% \midrule
% NCF              & 0.717 & 0.753 & 0.644 & 0.694 & 0.717 & 0.753 & 0.644 & 0.694 & 0.717 & 0.753 & 0.644 & 0.694 \\
% LGCN             & 0.722 & 0.718 & 0.730 & 0.724 & 0.717 & 0.753 & 0.644 & 0.694 & 0.717 & 0.753 & 0.644 & 0.694 \\
% LLM-Rec          & - & - & - & - & - & - & - & - & - & - & - & -\\
% InstructRec      & 0.769 & 0.833 & 0.672 & 0.744 & 0.717 & 0.753 & 0.644 & 0.694 & 0.717 & 0.753 & 0.644 & 0.694\\
% Tri-tower        & - & - & - & - & - & - & - & - & - & - & - & -\\
% \midrule
% BDLM-NCF-llm     & - & - & - & - & - & - & - & - & - & - & - & - \\
% BDLM-LGCN-llm    & - & - & - & - & - & - & - & - & - & - & - & - \\
% BDLM-NCF-drs      & 0.769 & 0.833 & 0.672 & 0.744 & 0.717 & 0.753 & 0.644 & 0.694 & 0.717 & 0.753 & 0.644 & 0.694\\
% BDLM-LGCN-drs      & 0.769 & 0.833 & 0.672 & 0.744 & 0.717 & 0.753 & 0.644 & 0.694 & 0.717 & 0.753 & 0.644 & 0.694\\

% \bottomrule

% \end{tabular}

% \caption{Main results on Math23k and the adapted MathQA test sets. "Acc(eq)" is the equation accuracy and "Acc(ans)" is the answer accuracy. "$*$" means our reimplementation based on released codes. "CL" is short for the contrastive learning. "mBERT" is short for the multilingual BERT.}
% \label{tab:main-res}
% \end{table*}

\begin{table*}[t]\small
\centering
\tabcolsep=0.18cm
\begin{tabular}{lcccccccccccc}
\toprule
Interaction Predict & \multicolumn{4}{c}{ML-1M} & \multicolumn{4}{c}{Grocery} & \multicolumn{4}{c}{Health} \\
Models & acc & prec & rec & f1 & acc & prec & rec & f1 & acc & prec & rec & f1 \\
\midrule
NCF              & 0.717 & 0.753 & 0.644 & 0.694 & 0.691 & 0.758 & 0.561 & 0.645 & 0.662 & 0.721 & 0.529 & 0.610 \\
LGCN             & 0.723 & 0.733 & 0.702 & 0.717 & 0.707 & 0.764 & 0.599 & 0.672 & 0.692 & 0.739 & 0.595 & 0.659 \\
LLM-Rec          & - & - & - & - & - & - & - & - & - \\
InstructRec      & 0.769 & 0.833 & 0.672 & 0.744 & 0.695 & 0.761 & 0.567 & 0.650 & 0.676 & 0.770 & 0.503 & 0.608 \\
Tri-tower        & - & - & - & - & - & - & - & - & - \\
\midrule
LLM-UIToken      & 0.770 & 0.826 & 0.684 & 0.748 & 0.695 & 0.753 & 0.579 & 0.655 & 0.677 & 0.768 & 0.506 & 0.610 \\
LLM-NCF          & 0.794 & 0.845 & 0.719 & 0.777 & 0.715 & 0.785 & 0.592 & 0.675 & 0.694 & 0.769 & 0.556 & 0.645 \\
LLM-LGCN         & 0.805 & 0.858 & 0.732 & 0.790 & 0.731 & 0.790 & 0.628 & 0.700 & 0.708 & 0.775 & 0.587 & 0.668 \\
\midrule
NCF-LLM          & 0.801 & 0.823 & 0.767 & 0.794 & 0.712 & 0.763 & 0.615 & 0.681 & 0.701 & 0.761 & 0.584 & 0.661 \\
LGCN-LLM         & 0.809 & 0.804 & 0.819 & 0.811 & 0.721 & 0.774 & 0.625 & 0.692 & 0.711 & 0.761 & 0.616 & 0.681 \\
\midrule
BDLM-NCF-LLM     & 0.801 & 0.839 & 0.745 & 0.789 & 0.714 & 0.776 & 0.600 & 0.677 & 0.695 & 0.767 & 0.561 & 0.648 \\
BDLM-LGCN-LLM    & 0.810 & 0.847 & 0.758 & 0.799 & 0.704 & 0.754 & 0.605 & 0.671 & 0.699 & 0.746 & 0.604 & 0.678 \\
BDLM-NCF-DRS     & 0.805 & 0.821 & 0.780 & 0.800 & 0.716 & 0.773 & 0.611 & 0.683 & 0.702 & 0.763 & 0.588 & 0.664 \\
BDLM-LGCN-DRS    & 0.815 & 0.812 & 0.819 & 0.816 & 0.725 & 0.777 & 0.631 & 0.697 & 0.716 & 0.750 & 0.616 & 0.681 \\

\bottomrule

\end{tabular}

\caption{Main results on MovieLens-1M, Amazon-Grocery and Amazon-Health test sets for interaction prediction task.}
\label{tab:main-res}
\end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}{llcccccc}
% \toprule
% ~ & ~ & \multicolumn{2}{c}{Top-K Reco} & \multicolumn{4}{c}{Interation Prediction} \\
% Dataset & Models & hr@1 & hr@2 & acc & prec & rec & f1  \\
% \midrule
% \multirow{7}*{ML-1M} &  NCF  & 0.251 & 0.416 & 0.717 & 0.753 & 0.644 & 0.694 \\
% ~ & LGCN                         & 0.284 & 0.448 & 0.722 & 0.718 & 0.730 & 0.724 \\
% ~ & LLM-Rec                      & - & - & - & - & - & - \\
% ~ & InstructRec                  & 0.372 & 0.483 & 0.769 & 0.833 & 0.672 & 0.744 \\
% ~ & Tri-tower                    & - & - & - & - & - & - \\
% ~ & BDLM-NCF-LLM               & 67.8 & 80.5 & 72.0 & 73.5 \\
% ~ & BDLM-NCF-DRS  & \textbf{70.9} & \textbf{83.9} & \textbf{74.2} & \textbf{76.3} \\
% ~ & BDLM-LGCN-LLM               & 67.8 & 80.5 & 72.0 & 73.5 \\
% ~ & BDLM-LGCN-DRS  & \textbf{70.9} & \textbf{83.9} & \textbf{74.2} & \textbf{76.3} \\
% \midrule

% \multirow{7}*{Grocery} &  NCF              & - & 69.5 & ~63.3$^*$ & ~70.4$^*$ \\
% ~ & LGCN             & - & 75.6 & ~68.9$^*$ & ~71.3$^*$ \\
% ~ & LLM-Rec          & - & 77.4 & ~70.0$^*$ & ~72.0$^*$ \\
% ~ & InstructRec      & 71.2 & 82.4 & 73.5 & 75.1 \\
% ~ & Tri-tower        & \textbf{71.8} & \textbf{83.2} & \textbf{74.4} & \textbf{76.3} \\
% ~ & BDLM-LLM               & 67.8 & 80.5 & 72.0 & 73.5 \\
% ~ & BDLM-DRS  & \textbf{70.9} & \textbf{83.9} & \textbf{74.2} & \textbf{76.3} \\
% \midrule

% \multirow{7}*{Health} &  NCF              & - & 69.5 & ~63.3$^*$ & ~70.4$^*$ \\
% ~ & LGCN             & - & 75.6 & ~68.9$^*$ & ~71.3$^*$ \\
% ~ & LLM-Rec          & - & 77.4 & ~70.0$^*$ & ~72.0$^*$ \\
% ~ & InstructRec      & 71.2 & 82.4 & 73.5 & 75.1 \\
% ~ & Tri-tower        & \textbf{71.8} & \textbf{83.2} & \textbf{74.4} & \textbf{76.3} \\
% ~ & BDLM-LLM               & 67.8 & 80.5 & 72.0 & 73.5 \\
% ~ & BDLM-DRS  & \textbf{70.9} & \textbf{83.9} & \textbf{74.2} & \textbf{76.3} \\
% \bottomrule

% \end{tabular}

% \caption{Main results on Math23k and the adapted MathQA test sets. "Acc(eq)" is the equation accuracy and "Acc(ans)" is the answer accuracy. "$*$" means our reimplementation based on released codes. "CL" is short for the contrastive learning. "mBERT" is short for the multilingual BERT.}
% \label{tab:main-res}
% \end{table*}

==> Tables/main-res2.tex <==
% \begin{table*}[t]
% \centering
% \begin{tabular}{lcccccccccccc}
% \toprule
% Interaction Predict & \multicolumn{4}{c}{ML-1M} & \multicolumn{4}{c}{Grocery} & \multicolumn{4}{c}{Health} \\
% Models & acc & prec & rec & f1 & acc & prec & rec & f1 & acc & prec & rec & f1 \\
% \midrule
% NCF              & 0.717 & 0.753 & 0.644 & 0.694 & 0.717 & 0.753 & 0.644 & 0.694 & 0.717 & 0.753 & 0.644 & 0.694 \\
% LGCN             & 0.722 & 0.718 & 0.730 & 0.724 & 0.717 & 0.753 & 0.644 & 0.694 & 0.717 & 0.753 & 0.644 & 0.694 \\
% LLM-Rec          & - & - & - & - & - & - & - & - & - & - & - & -\\
% InstructRec      & 0.769 & 0.833 & 0.672 & 0.744 & 0.717 & 0.753 & 0.644 & 0.694 & 0.717 & 0.753 & 0.644 & 0.694\\
% Tri-tower        & - & - & - & - & - & - & - & - & - & - & - & -\\
% \midrule
% BDLM-NCF-llm     & - & - & - & - & - & - & - & - & - & - & - & - \\
% BDLM-LGCN-llm    & - & - & - & - & - & - & - & - & - & - & - & - \\
% BDLM-NCF-drs      & 0.769 & 0.833 & 0.672 & 0.744 & 0.717 & 0.753 & 0.644 & 0.694 & 0.717 & 0.753 & 0.644 & 0.694\\
% BDLM-LGCN-drs      & 0.769 & 0.833 & 0.672 & 0.744 & 0.717 & 0.753 & 0.644 & 0.694 & 0.717 & 0.753 & 0.644 & 0.694\\

% \bottomrule

% \end{tabular}

% \caption{Main results on Math23k and the adapted MathQA test sets. "Acc(eq)" is the equation accuracy and "Acc(ans)" is the answer accuracy. "$*$" means our reimplementation based on released codes. "CL" is short for the contrastive learning. "mBERT" is short for the multilingual BERT.}
% \label{tab:main-res}
% \end{table*}

\begin{table*}[h]\small
\centering
\begin{tabular}{lcccccc}
\toprule
Top-K Recommendation & \multicolumn{2}{c}{ML-1M} & \multicolumn{2}{c}{Grocery} & \multicolumn{2}{c}{Health} \\
Models & hr@1 & hr@2 & hr@1 & hr@2 & hr@1 & hr@2 \\
\midrule
NCF              & 0.251 & 0.416 & 0.265 & 0.439 & 0.251 & 0.399  \\
LGCN             & 0.284 & 0.448 & 0.337 & 0.516 & 0.344 & 0.481  \\
LLM-Rec          & - & - & - & - & - & - \\
InstructRec      & 0.372 & 0.483 & 0.339 & 0.437 & 0.309 & 0.358  \\
Tri-tower        & - & - & - & - & - & - \\
\midrule
LLM+UIToken      & 0.312 & 0.361 & 0.310 & 0.374 & 0.321 & 0.375  \\
LLM+NCF          & 0.398 & 0.523 & 0.387 & 0.474 & 0.331 & 0.431  \\
LLM+LGCN         & 0.431 & 0.545 & 0.373 & 0.458 & 0.380 & 0.466  \\
\midrule
NCF+LLM          & 0.405 & 0.584 & - & - & - & -  \\
LGCN+LLM         & 0.460 & 0.607 & - & - & - & -  \\

\bottomrule

\end{tabular}

\caption{Main results on MovieLens-1M, Amazon-Grocery and Amazon-Health test sets for top-K recommendation task.}
\label{tab:main-res2}
\end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}{llcccccc}
% \toprule
% ~ & ~ & \multicolumn{2}{c}{Top-K Reco} & \multicolumn{4}{c}{Interation Prediction} \\
% Dataset & Models & hr@1 & hr@2 & acc & prec & rec & f1  \\
% \midrule
% \multirow{7}*{ML-1M} &  NCF  & 0.251 & 0.416 & 0.717 & 0.753 & 0.644 & 0.694 \\
% ~ & LGCN                         & 0.284 & 0.448 & 0.722 & 0.718 & 0.730 & 0.724 \\
% ~ & LLM-Rec                      & - & - & - & - & - & - \\
% ~ & InstructRec                  & 0.372 & 0.483 & 0.769 & 0.833 & 0.672 & 0.744 \\
% ~ & Tri-tower                    & - & - & - & - & - & - \\
% ~ & BDLM-NCF-LLM               & 67.8 & 80.5 & 72.0 & 73.5 \\
% ~ & BDLM-NCF-DRS  & \textbf{70.9} & \textbf{83.9} & \textbf{74.2} & \textbf{76.3} \\
% ~ & BDLM-LGCN-LLM               & 67.8 & 80.5 & 72.0 & 73.5 \\
% ~ & BDLM-LGCN-DRS  & \textbf{70.9} & \textbf{83.9} & \textbf{74.2} & \textbf{76.3} \\
% \midrule

% \multirow{7}*{Grocery} &  NCF              & - & 69.5 & ~63.3$^*$ & ~70.4$^*$ \\
% ~ & LGCN             & - & 75.6 & ~68.9$^*$ & ~71.3$^*$ \\
% ~ & LLM-Rec          & - & 77.4 & ~70.0$^*$ & ~72.0$^*$ \\
% ~ & InstructRec      & 71.2 & 82.4 & 73.5 & 75.1 \\
% ~ & Tri-tower        & \textbf{71.8} & \textbf{83.2} & \textbf{74.4} & \textbf{76.3} \\
% ~ & BDLM-LLM               & 67.8 & 80.5 & 72.0 & 73.5 \\
% ~ & BDLM-DRS  & \textbf{70.9} & \textbf{83.9} & \textbf{74.2} & \textbf{76.3} \\
% \midrule

% \multirow{7}*{Health} &  NCF              & - & 69.5 & ~63.3$^*$ & ~70.4$^*$ \\
% ~ & LGCN             & - & 75.6 & ~68.9$^*$ & ~71.3$^*$ \\
% ~ & LLM-Rec          & - & 77.4 & ~70.0$^*$ & ~72.0$^*$ \\
% ~ & InstructRec      & 71.2 & 82.4 & 73.5 & 75.1 \\
% ~ & Tri-tower        & \textbf{71.8} & \textbf{83.2} & \textbf{74.4} & \textbf{76.3} \\
% ~ & BDLM-LLM               & 67.8 & 80.5 & 72.0 & 73.5 \\
% ~ & BDLM-DRS  & \textbf{70.9} & \textbf{83.9} & \textbf{74.2} & \textbf{76.3} \\
% \bottomrule

% \end{tabular}

% \caption{Main results on Math23k and the adapted MathQA test sets. "Acc(eq)" is the equation accuracy and "Acc(ans)" is the answer accuracy. "$*$" means our reimplementation based on released codes. "CL" is short for the contrastive learning. "mBERT" is short for the multilingual BERT.}
% \label{tab:main-res}
% \end{table*}

==> Tables/prompt.tex <==
\begin{table}[t]
\centering
\small

\begin{tabular}{p{0.18\linewidth}p{0.48\linewidth}c}
\toprule
Task & Instruction & Answer\\
\midrule
Interaction & Prediction User has watched the following movies (A Close Shave), (Aladdin)... Predict if he/she will watch (Pocahontas)next. Answer: & Yes\\
\midrule
Interaction Prediction & \yellowbox{User} \red{<uid1>} has watched the following movies \red{<iid745>} (A Close Shave), \red{<iid588>} (Aladdin)... Predict if he/she will watch \red{<iid48>} (Pocahontas) next. Answer: & Yes\\
\bottomrule
\end{tabular}

\caption{The prompt format of interaction prediction task and top-K recommendation task.}
\label{tab:prompt}
\end{table}
